Interstellar Complex Organic Molecules in SiO-traced massive outflows

The interstellar medium contains dust and gas, in which at high densities and cold conditions molecules can proliferate. Interstellar Complex Organic Molecules (iCOMs) are C-bearing species that contain at least six atoms. As they are detected in young stellar objects, iCOMs are expected to inhabit the early stages of the star formation evolution. In this study, we try to determine which iCOMs are present in the outflow component of massive protostars. To do this, we analyzed the morphological extension of blue- and red-shifted iCOMs emission in a sample of eleven massive protostars employing mapping observations at one mm within a ~1 GHz bandwidth for both IRAM-30m and APEX telescopes. We modeled the iCOMs emission of the central pointing spectra of our objects using the XCLASS LTE radiative transfer code. We detected the presence of several iCOMs such as: CH3OH, 13CH3OH, CH3OCHO, C2H5C15N, and c-C3H2)CH2. In G034.41+0.24, G327.29-0.58, G328.81+0.63, G333.13-0.43, G340.97-1.02, G351.45+0.66 and G351.77-0.54, the iCOMs lines show a faint broad line profile. Due to the offset peak positions of the blue- and red-shifted emission, covering from ~0.1 to 0.5 pc, these wings are possibly related to movements external to the compact core, such as large-scale low-velocity outflows. We have also established a correlation between the parent iCOM molecule CH3OH and the shock tracer SiO, reinforcing the hypothesis that shock environments provide the conditions to boost the formation of iCOMs via gas-phase reactions.

==> Tables/chisquere.tex <==
 \begin{table}[!htpb]
	\centering
	\caption{Results for the $\chi^2$ test for the models into our sample. The second column display the degrees of freedom of the data using n-1 with n = channels into each source. The third column shows the critical value of $\chi^2$ to reach the p-value of 0.05. The fourth column shows the computed model vs data $\chi^2$ test. (*) This source have not pass the significance p-value of 0.05 threshold, as their observational data was the noisiest one, due to the worst observation conditions (tau=0.3).}
		%\footnotesize 
	\begin{tabular}{cccccccccc}
		%\tabletypesize{\scriptsize}
		\toprule
Source & DF & Crit $\chi^2$ & $\chi^2$ \\
\midrule  
G034.26+0.15	&	283	&	324.31	&	8.21	\\
G034.41+0.24	&	283	&	324.31	&	3.54	\\
G035.13-0.74	&	383	&	429.63	&	7.53	\\
G327.29-0.58	&	360	&	406.30	&	28.25	\\  Better
G328.81+0.63	&	360	&	406.30	&	23.56	\\ Wrong
G333.13-0.43	&	360	&	406.30	&	14.34	\\
G337.92-0.48	&	360	&	406.30	&	60.53	\\
G340.97-1.02*	&	360	&	406.30	&	559.68	\\
G351.45+0.66	&	360	&	406.30	&	72.27	\\
G351.77-0.54	&	360	&	406.30	&	162.16	\\
G353.41-0.36	&	360	&	406.30	&	53.83	\\
\bottomrule                                                  
\end{tabular}\label{chisquere_Table}
\end{table}  


==> Tables/delta_v.tex <==
\begin{table*}[!htpb]
	\centering
	\caption{Integration intervals over each molecule line emission for all of our sources. ($^{*}$) This emission range is mainly dominated by the strong DCN emitter.}
		%\footnotesize 
	\begin{tabular}{cccccccccccccc} 
		%\tabletypesize{\scriptsize}
		\toprule
 \multirow{2}*{Molecule} &  Frequency  & G327.29-0.58 & G328.81+0.63  & G333.13-0.43 & G337.92-0.48 & G340.97-1.02 & G351.45+0.66 \\                                                                                                        
    &    (GHz)    & [Kms$^{-1}$] &  [Kms$^{-1}$] &  [Kms$^{-1}$]  &  [Kms$^{-1}$]   &  [Kms$^{-1}$]  &  [Kms$^{-1}$]      \\                                                  
\midrule                    
CH$_3$OCHO          &  216.830197	&   5.34	&    ---	&   ---	&   ---	&---	&---   \\
CH$_3$OCHO       	&  216.838889	&   11.34	&    ---	&   ---	&   ---	&---	&---   \\
CH$_3$OH            &  216.945559	&   8.34	&    8.27	&   5.59	&   5.59	&8.32	&8.32  \\
CH$_3$OCHO          &  216.965900	&   10.95	&    5.58	&   ---	&   ---	&---	&---   \\
CH$_3$OCHO          &  216.967994	&   10.95	&    ---	&   11.04	&   3.15	&---	&8.32  \\
SiO         	    &  217.104984	&   10.95	&    19.14	&   16.92	&   16.63	&5.74	&16.63 \\
C$_2$H$_5$CN$^{15}$ &  217.190187	&   8.34	&    ---	&   ---	&   ---	&---	&---   \\
CH$_3$OCHO$^{*}$     	&  217.237558	&   5.48	&    8.27	&   8.32	&   8.03	&---	&8.17  \\
CH$_3$OCHO      	&  217.298353	&   8.21	&    ---	&   ---	&   ---	&---	&8.03  \\
CH$_3$OCHO          &  217.301326	&   ---	&    ---	&   10.90	&   2.72	&---	&---   \\
$^{13}$CH$_3$OH     &  217.399550	&   ---	&    ---	&   ---	&   ---	&---	&---   \\
CH$_3$OH       	    &  217.418711	&   ---	&    ---	&   ---	&   ---	&---	&---   \\
($c-$C$_3$H$_2$)CH$_2$&  217.429650	&   ---	&    ---	&   ---	&   ---	&---	&5.16  \\
\midrule
 \multirow{2}*{Molecule} &  Frequency  & G351.77-0.54 & G353.41-0.36 & G35.13-0.74 & G34.41+0.24 & G34.26+0.15 \\                                                                                                        
                         &    (GHz)    & [Kms$^{-1}$] &  [Kms$^{-1}$] & [Kms$^{-1}$] & [Kms$^{-1}$] &   [Kms$^{-1}$]     \\                                                  
\midrule 
CH$_3$OCHO          &  216.830197	& ---	& ---	& ---	& ---	& ---    \\
CH$_3$OCHO       	&  216.838889	& ---	& ---	& ---	& ---	& ---    \\
CH$_3$OH            &  216.945559	& 10.98	& ---	& ---	& 11.21	& 5.22   \\
CH$_3$OCHO          &  216.965900	& ---	& ---	& ---	& 8.21	& ---    \\
CH$_3$OCHO          &  216.967994	& 8.46	& ---	& ---	& 8.21	& ---    \\
SiO         	    &  217.104984	& 27.82	& 8.17	& 8.08	& 13.82	& 10.61  \\
C$_2$H$_5$CN$^{15}$ &  217.190187	& ---	& ---	& ---	& ---	& ---    \\
CH$_3$OCHO$^{*}$      	&  217.237558	& 13.79	& 5.88	& 7.94	& 8.34	& 8.35   \\
CH$_3$OCHO      	&  217.298353	& ---	& ---	& ---	& 10.82	& ---    \\
CH$_3$OCHO          &  217.301326	& 8.32	& ---	& ---	& ---	& ---    \\
$^{13}$CH$_3$OH     &  217.399550	& 5.31	& ---	& ---	& ---	& ---    \\
CH$_3$OH       	    &  217.418711	& 8.43	& ---	& ---	& ---	& ---    \\
($c-$C$_3$H$_2$)CH$_2$&  217.429650	& ---	& ---	& ---	& ---	& ---    \\
\bottomrule                                                  
\end{tabular}\label{Delta_v}
\end{table*}  


==> Tables/table_CD.tex <==
\begin{table*}[!htpb]
	\centering
	\caption{Column density computed using the classical LTE aproximation method. This were used to compute the Rotational diagrams into our sample. This values are the consequence of the T$_{Mb}$ reported into Table \ref{Tmb_Int}.}
	\footnotesize 
	\begin{tabular}{cccccccccccccc} 
		%\tabletypesize{\scriptsize}
		\toprule
 \multirow{2}*{Molecule} &  Frequency  & G327.29-0.58 & G328.81+0.63  & G333.13-0.43 & G337.92-0.48 & G340.97-1.02  \\                                                                                                        
    &    (GHz)           &  Nu [cm$^{-2}$]  & Nu [cm$^{-2}$] &  Nu [cm$^{-2}$] & Nu [cm$^{-2}$] & Nu [cm$^{-2}$]    \\                                                  
\midrule                    
CH$_3$OCHO          &  216.830197	&1.20E12$\pm$1.55E11  & ---                    & ---                 & ---                  & ---                   \\
CH$_3$OCHO       	&  216.838889	&2.57E12$\pm$2.38E11  & ---                    & ---                 & ---                  & ---                   \\
CH$_3$OH            &  216.945559	&6.50E13$\pm$5.72E12  & 3.78E13$\pm$1.53E12  & 1.92E13$\pm$1.08E12 & 2.09E13$\pm$2.51E12 & 1.43E13$\pm$3.83E12 \\
CH$_3$OCHO          &  216.965900	&4.27E12$\pm$3.35E11  & 6.17E11$\pm$8.64E10  & ---                 & ---                  & ---                  \\
CH$_3$OCHO          &  216.967994	& ---  & ---                    & 4.81E12$\pm$8.59E11 & 2.01E12$\pm$6.90E11 & ---                 \\
SiO         	    &  217.104984	&1.60E12$\pm$3.74E10  & 3.00E12$\pm$8.12E10  & 1.35E12$\pm$5.07E10 & 2.03E12$\pm$1.02E11 & 9.34E11$\pm$6.68E10 \\
C$_2$H$_5$CN$^{15}$ &  217.190187	&5.30E12$\pm$5.03E11  & ---                    & ---                 & ---                  & ---                   \\
CH$_3$OCHO      	&  217.237558	&1.64E15$\pm$7.77E13  & 2.41E15$\pm$6.23E13  & 9.34E14$\pm$6.04E13 & 1.76E15$\pm$7.98E13 & ---                   \\
CH$_3$OCHO      	&  217.298353	&2.07E15$\pm$1.23E14  & ---                    & ---                 & ---                  & ---                   \\
CH$_3$OCHO          &  217.301326	&---                  & ---                      & 5.88E14$\pm$6.69E13 & 1.19E14$\pm$5.01E13 & ---                   \\
$^{13}$CH$_3$OH     &  217.399550	&---                  & ---                      & ---                 & ---                  & ---                   \\
CH$_3$OH       	    &  217.418711	&---                  & ---                      & ---                 & ---                  & ---                   \\
($c-$C$_3$H$_2$)CH$_2$&  217.429650	&---                  & ---                      & ---                 & ---                  & ---                   \\
\midrule  
 \multirow{2}*{Molecule}   & G351.45+0.66 & G351.77-0.54 & G353.41-0.36 & G35.13-0.74 & G34.41+0.24 & G34.26+0.15 \\                       
                           &   Nu [cm$^{-2}$]  & Nu [cm$^{-2}$] &  Nu [cm$^{-2}$] & Nu [cm$^{-2}$] & Nu [cm$^{-2}$] &   Nu [cm$^{-2}$]     \\   
\midrule  
CH$_3$OCHO               & ---                 & ---                  & ---                   & ---                   & ---                   & --- \\
CH$_3$OCHO       	     & ---                 & ---                  & ---                   & ---                   & ---                   & --- \\
CH$_3$OH                 & 3.95E13$\pm$1.41E12 & 5.03E13$\pm$2.93E12 & ---                   & ---                   & 3.51E13$\pm$9.43E11 & 5.56E12$\pm$9.28E11 \\
CH$_3$OCHO               & ---                 & ---                  & ---                   & ---                   & 1.40E12$\pm$6.34E10 & --- \\
CH$_3$OCHO               & 5.31E12$\pm$7.84E11 & 1.31E13$\pm$1.30E12 & ---                   & ---                   & ---  & --- \\
SiO         	         & 3.27E12$\pm$1.13E11 & 5.51E12$\pm$2.97E11 & 8.64E11$\pm$4.43E10 & 4.03E11$\pm$1.80E10 & 1.54E12$\pm$3.46E10 & 7.28E11$\pm$3.22E10 \\
C$_2$H$_5$CN$^{15}$      & ---                 & ---                  & ---                   & ---                   & ---                   & --- \\
CH$_3$OCHO      	     & 1.75E15$\pm$6.06E13 & 4.00E15$\pm$1.23E14 & 6.30E14$\pm$8.49E13 & 5.92E14$\pm$3.50E13 & 1.48E15$\pm$3.75E13 & 6.29E14$\pm$3.98E13 \\
CH$_3$OCHO      	     & 4.39E14$\pm$8.76E13 & ---                  & ---                   & ---                   & 1.06E15$\pm$4.26E13 & --- \\
CH$_3$OCHO               & ---                 & 9.59E14$\pm$9.69E13 & ---                   & ---                   & ---                   & --- \\
$^{13}$CH$_3$OH          & ---                 & 1.32E13$\pm$1.17E12 & ---                   & ---                   & ---                   & --- \\
CH$_3$OH       	         & ---                 & 2.27E19$\pm$2.87E18 & ---                   & ---                   & ---                   & --- \\
($c-$C$_3$H$_2$)CH$_2$   & 3.27E13$\pm$1.13E13 & ---                   & ---                   & ---                   & ---                   & --- \\
\bottomrule                                                  
\end{tabular}\label{Table_CD}
\end{table*}  


==> Tables/table_trot.tex <==
 \begin{table}[!htpb]
	\centering
	\caption{Rotational temperature gathered toward objects in our sample whit at least two transitions of Methyl Formade (CH$_3$OCHO).  The third column displays the $\sigma_{T_{Rot}}$ corresponding to the error due to linear regression. (*) Not significant error due to a just two point fit.}
		%\footnotesize 
	\begin{tabular}{ccccccccccccccccc}
		%\tabletypesize{\scriptsize}
		\toprule
 \multirow{2}*{Molecule}   & $T_{rot}$ &     $\sigma_{T_{rot}}$\\
                   & [K]       &       [K]             \\
\midrule  
G327.29-0.58               &  27.23      &  4.25              \\
G328.81+0.63               &  22.07       &  2.69E-42*  \\              
G333.13-0.43               &  33.89      &   2.15             \\
G337.92-0.48               &  31.90      &   11.02              \\
G351.45+0.66               &  30.70       &  1.48               \\
G351.77-0.54               &  34.07      &   6.75             \\
G34.41+0.24                &  24.57     &    2.57              \\
\bottomrule                                                  
\end{tabular}\label{t_rot_Table}
\end{table}  













                                 	
                                 	
                                 	
                                 	
                                 	
                                 	
                                 	




==> Tables/xclass_simple_mol.tex <==
\begin{table*}[!htpb]
	\centering
	\caption{Results of the XCLASS modeling for the found simple molecules}
	%	\footnotesize 
	\begin{tabular}{ccccccccccccccccc}
		%\tabletypesize{\scriptsize}
		\toprule
		 \multirow{3}*{Source} & T$_{rot}$ & N$_{Tot}$  & $\Delta v$&    \multirow{3}*{Source} &  T$_{rot}$ & N$_{Tot}$  & $\Delta v$\\
		                       & [K]       & [cm$^{-2}$] & kms$^{-1}$&                           &  [K]       & [cm$^{-2}$] & kms$^{-1}$\\
		\cmidrule(r){2-4}                                                 \cmidrule(r){6-8} 
		                       &\multicolumn{3}{c}{SiO;v=0 (Narrow)}      &     & \multicolumn{3}{c}{SiO;v=0 (Wide)}      \\
		\midrule
        G034.26+0.15     &	61.611	&	5.19E+12	&	6.04	& G034.26+0.15	&	84.967	&	8.44E+12	&	21.88 \\
        G034.41+0.24     &  120.000	&	6.59E+12	&	5.62	& G034.41+0.24	&	216.148	&	2.63E+13	&	21.02 \\
        G035.13-0.74     &	79.695	&	5.50E+12	&	7.20	& G035.13-0.74	&	400.004	&	1.00E+13	&	28.13 \\
        G327.29-0.58     &	19.582	&	2.72E+13	&	5.68	& G327.29-0.58	&	100.924	&	1.01E+13	&	18.21 \\
        G328.81+0.63     &	151.685	&	7.42E+12	&	5.21	& G328.81+0.63    &	16.635	&	6.55E+13	&	10.00\\
        G333.13-0.43     &	28.798	&	1.02E+13	&	6.57	& G333.13-0.43	&	188.425	&	2.20E+13	&	20.62 \\
        G337.92-0.48     &	89.486	&	3.94E+13	&	8.96	& G337.92-0.48	&	33.442	&	1.18E+13	&	40.57 \\
        G340.97-1.02     &	33.230	&	1.82E+13	&	7.11	& G340.97-1.02	&	27.929	&	8.66E+12	&	23.94 \\   
        G351.45+0.66     &	85.160	&	5.17E+13	&	5.96	& G351.45+0.66	&	31.786	&	1.83E+13	&	28.00 \\
        G351.77-0.54     &	17.839	&	5.41E+13	&	7.69	& G351.77-0.54	&	32.781	&	3.67E+13	&	34.12 \\
        G353.41-0.36     &	21.318	&	1.50E+13	&	6.75	& G353.41-0.36	&	52.822	&	7.42E+12	&	31.91 \\
		\midrule
		Source     &\multicolumn{3}{c}{DCN;v=0}      & Source    & \multicolumn{3}{c}{HCCC$^{13}$N;v=0}      \\
		\midrule
        G034.26+0.15	 &	61.844	&	2.13E+12	&	3.21 &  G327.29-0.58	&	11.463	&	4.47E+16	&	1.12     \\
        G034.41+0.24	 &	340.768	&	1.51E+13	&	5.72 &  G337.92-0.48	&	13.926	&	8.17E+15	&	10.00     \\
        G035.13-0.74	 &	126.094	&	3.05E+12	&	3.53 &  G351.77-0.54	&	16.735	&	5.45E+15	&	14.84     \\
        G328.81+0.63	 &	300.617	&	5.96E+13	&	4.32 &               &           &               &     \\
        G333.13-0.43	 &	307.719	&	2.20E+13	&	4.48 &               &           &               &           \\   
        G337.92-0.48	 &	54.482	&	1.04E+13	&	5.25 &               &           &               &          \\
        G340.97-1.02	 &	141.166	&	8.01E+12	&	4.49 &               &           &               &          \\
        G351.45+0.66	 &	161.847	&	2.20E+13	&	2.83 &               &           &               &          \\
        G353.41-0.36	 &	362.937	&	2.28E+13	&	4.62 &               &           &               &          \\
		\midrule
		Source     &\multicolumn{3}{c}{$t-$HC$_3$O;v=0}      & Source    & \multicolumn{3}{c}{C$^{13}$CC$^{13}$S}      \\
		\midrule
          G327.29-0.58	&	499.969	&	1.27E+16	&	14.32   & G034.26+0.15	&	208.972	&	4.34E+12	&	5.19  \\
          G351.45+0.66	&	54.532	&	2.21E+15	&	2.69    & G035.13-0.74	&	208.604	&	6.94E+12	&	3.97  \\
		\midrule
		Source     &\multicolumn{3}{c}{C$_3$H;v=0}       &           &         &      &    \\
		\midrule		
        G327.29-0.58	&	60.063	&	6.89E+17	&	6.00             &  & 	& 	&  \\
		\bottomrule                                                  
	\end{tabular}\label{simple_Mol_xclass_result}
\end{table*} 
